Cut-Cell Microstructures for Two-scale Structural Optimization

Two-scale topology optimization, combined with the design of microstructure families with a broad range of effective material parameters, is increasingly widely used in many fabrication applications to achieve a target deformation behavior for a variety of objects. The main idea of this approach is to optimize the distribution of material properties in the object partitioned into relatively coarse cells, and then replace each cell with microstructure geometry that mimics these material properties. In this paper, we focus on adapting this approach to complex shapes in situations when preserving the shape's surface is important. Our approach extends any regular (i.e. defined on a regular lattice grid) microstructure family to complex shapes, by enriching it with individually optimized cut-cell tiles adapted to the geometry of the cut-cell. We propose an automated and robust pipeline based on this approach, and we show that the performance of the regular microstructure family is only minimally affected by our extension while allowing its use on 2D and 3D shapes of high complexity.

==> 32-homogenization.tex <==

\subsection{Construction of $\mtg$}
\label{sec:hom}

We use the method introduced in \cite{tozoni2020low} for creating low-parametric microstructure families for the interior cells both for 2D and 3D (\cite{tozoni2020low} is focused primarily on 2D). However, we do not use their rhombic shape parameter, as in our case we will use only square/cubic cells.

First, \emph{a homogenization map}  $H(\p)$  is obtained for a low-parametric family of microstructures, with parameters shown in Figure~\ref{fig:parameters}, consisting of graph vertex positions and radii at these vertices determining how thick the microstructure is at this location.  

 For each shape parameter, we consider a range $[p^{min}_i, p^{max}_i]$ determined by geometric constraints: vertex positions need to remain within the cell with some constrained to the boundary, and radii at vertices are  $B_p$ is the  $n$-dimensional box of admissible parameter values. %

We run a sweep of the parameter values in these ranges. Each combination of values is used to generate a microstructure cell geometry using the implicit surface definition of \cite{Panetta:2017:WCS}.   The value of $H(\p)$ is obtained as the effective value of the elasticity tensor parameters (with additional symmetry conditions on our structures there are only 3 independent parameters in the tensor, Young's modulus $E$, Poisson's ratio $\nu$ and the shear modulus $G)$, so the function $H(\p)$ maps $\p$ into $\reals^3$. 

The map $H(\p)$ is not bijective as it typically maps a higher-dimensional space into a lower-dimensional space.  In  \cite{tozoni2020low}, a sequence of dimension reductions is used to identify a subspace $D$ in the space of shape parameters equal to the dimension of the elasticity material parameter space (3 in our case). 
The map $H(\p)$ restricted to this subspace may still be not bijective, but its image $H(B_p)$ can be partitioned into parts on which it is invertible; specifically, we construct simplexes in the subspace of shape parameters 
and  split $B_p \cap D$ into connected subdomains $D_j$ by simplex orientation. 
On each of $D_j$, we can invert $H(\p)$.  We further restrict it to the 
two-dimensional space of isotropic material parameters parametrized by $(E,\nu)$
to obtain the  \emph{material-to-geometry} map $\mtg_i(E,\nu): D_i \rightarrow  B^p$. 

Figure~\ref{fig:coverage} presents the coverage regions for our 2D and 3D families. Notice that for 3D we have two different material coverage sheets, with the red one covering most of the space and being chosen as our main material range.

\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.35\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/coverage_2D.pdf}
        \caption{2D}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{0.35\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/coverage_3D.pdf}
        \caption{3D}
    \end{subfigure}
    \caption{Coverage of material parameter properties in the families we use. Our coverage regions are approximated to triangles, so they can be easily added as constraints in our optimization.}
\label{fig:coverage}
\end{figure}

Figure~\ref{fig:shape-param} shows examples on the final map from material properties ($\nu$ and $E$) to geometric parameters $p_i$. 

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{images/shape-param.pdf}
    \caption{Examples of shape parameter dependence on materials in our 3D family. For illustration purposes, we display maps for parameters $p_1$, $p_2$ and $p_8$, but there are similar maps for all of our $8$ parameters. These maps correspond to our main coverage sheet.}
    \label{fig:shape-param}
\end{figure}


==> 33-boundary-cells.tex <==
\subsection{Microstructure for cut cells}
\label{sec:cutcells}

The main difficulty of the cut-cell approach is that the boundary cells may have unpredictable shapes and are generally not amenable to the homogenization approach that we use for cubic cells. Cut-cells cannot be tiled periodically in a way that reflects their behavior in the real structure, as these are always attached to the boundary. 

We aim to design a way to handle the cells overlapping the boundary, that allows us to retain control over their effective material properties while satisfying the necessary geometric constraints. 

We start with the most obvious solutions, one of which we use as a baseline for our method.  The two options requiring the fewest changes to already existing pipelines for handling the cut cells are (1) to cut the standard interior-cell microstructure \cite{schumacher2015microstructures} \DP{Check me, and add more if there are} and (2) to fill the cell with solid material.%

The downsides of the first approach are obvious: arbitrarily cutting a microstructure may result in dramatic uncontrollable changes in the effective material properties, as well as entirely disconnected structures, and the resulting object has no surface layer which may be needed for its function. 

The second approach ensures that any microstructure can be used in the interior and that the object has a solid surface. However, it provides no control over the behavior of the cells near the boundary. 

Our approach aims to recover some of the desirable properties of the microstructure design while retaining the desirable properties of fully filled cells, i.e., the support for an (almost everywhere) solid surface, and  the ability to connect to any other microstructure in the interior. 

We found that  creating voids of adjustable size in the boundary cells already 
yields a significant improvement compared to fully solid cells when combined with the additional optimization step we discussed in the overview. 

For a cell with a polygonal boundary $P$, we use a 1-parametric family of 
cells with the material filling the space between two nonintersecting polylines or surfaces $P$ and $P(r)$, where $r= r_{\min}\ldots 1$  is a parameter
interpolating between the minimal wall thickness and a fully filled cell. 
In 3D, we may need to add additional openings to avoid enclosed voids, as discussed in Section \ref{sec:tunnels}. The parameter $r$ is the volume fraction of the solid material in the resulting cell.  

While more complex constructions may allow for improved accuracy, we found that this construction already improves it by a large factor, for a negligible computational overhead compared to a standard two-scale method. 






We construct offsets using a signed distance function (SDF).  First, the cell boundary mesh is converted to an SDF (we use \cite{tao2019mandoline} in 2D and OpenVDB \cite{Museth:2013} for 3D).
This representation allows us to extract the approximate offset at any distance $d$ from the boundary. As the area/volume of the enclosed offset surface cannot be easily computed, we use a binary search to find a value of $d$ yielding an approximation of the desired volume with a relative tolerance $0.01$.

\begin{figure}
    \centering
    \includegraphics[width=0.65\linewidth]{images/boundary_cells/boundary-cells.pdf}
    \caption{Four examples of boundary cell geometry; the example on the right shows tunnels for material removal added.}
    \label{fig:boundary-cell}
\end{figure}

\paragraph{From volume fraction to material properties.}  We use a simplified material property model, as we correct the result by an additional optimization iteration, and assume that the boundary with the geometry described above can be approximated by a constant Poisson's ratio equal to the base material Poisson's ratio, the Young modulus is considered to be a function of the volume ratio, and the elasticity tensore is close to isotropic. 

The relationship between the effective Young's modulus and volume ratio, in general, depends on the shape of the cell, and in the case of non-tileable cells may even be difficult to define precisely, as it is unclear how to perform correct homogenization in this case.  However, a rough approximation of this dependence can be obtained from a one-parametric of cells, without boundary cuts. In this case, we can vary the internal void shape, and observe that the dependence on the shape of the void is not strong (Figure~\ref{fig:volume-Y}).
\DZ{TODO: still need this graph} We emphasize that we do not aim for precision, as we perform additional optimization with actual cell geometry in place.

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.45\columnwidth}
        \centering
        \includegraphics[width=1.0\columnwidth]{images/volume-Y.pdf}
        \caption{2D}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/volume-Y_3D.pdf}
        \caption{3D}
    \end{subfigure}
    \caption{Volume ratio to average Young's modulus map. In the left figure, each color represents a different shape of the opening.}
    \label{fig:volume-Y}
\end{figure}









==> 34-optimization.tex <==
\subsection{Material Optimization}
\label{sec:optimization}

In contrast to previously proposed two-scale methods, our optimization process includes two separate stages.  The first stage is standard material optimization. 

For all examples, we solve the problem with the following simple functional defined as follows:

\begin{equation}
    E(\u) = \int_{\partial \Omega^t} (\u - \u^0)^2 dA  + w \int_{\Omega \setminus \Omega^f} 
    \|\nabla C\|^2 dA
\end{equation}
where $\partial \Omega^t$ is typically a part of the boundary of our domain for which we prescribe target displacements. The constraints on the problem consist of a set of
linear bounds for the domain of realizable material properties shown in Figure~\ref{fig:coverage} for interior cells and a lower bound on the Young's modulus corresponding to the minimal allowed wall thickness for the boundary cells. 

At the second stage, the same process is applied to the mesh with microstructure geometry inserted for boundary cells; in this case, the material on the smaller-scale tetrahedral mesh for the microstructure of these cells is kept constant, so while the overall complexity of the optimization increases, as the simulation needs to be done on a finer mesh, it is still much lower than the complexity of direct  microstructure shape or topology optimization.  

\DZ{is this the regularization we use?  how is the gradient discretized? need to define parameters}
The problem is discretized using the finite element method, and the adjoint method is used to compute the gradient of the target functional with respect to elasticity parameters. The optimization itself is performed using L-BFGS. 
\DZ{information on convergence, should we include a plot? any other important details on optimization?}



==> 35-geometry.tex <==
\subsection{Geometric operations}
\label{sec:geometry} 

Our algorithm requires three geometric discretizations: (1) for step 1, it requires a relatively coarse volumetric mesh used by the material optimization, (2) for step 5, it requires a second volumetric mesh, with fine elements on the boundary to capture the boundary cell geometry, and (3) for step 7, it extracts a surface mesh of the optimized structure.

For the sake of clarity, we present the 3D construction first, and we briefly overview the difference with the 2D pipeline at the end of this section.

\paragraph{Cut-Cell Volumetric Meshing.}

The input is a surface mesh and a background regular grid, each grid corresponding to a microstructure tile. The output is a tetrahedral mesh of the interior of the surface mesh, with the regular grid represented as a collection of tetrahedral faces. This mesh is used for the first material optimization (Section \ref{sec:optimization}).

This problem could be solved by computing a 3D arrangement \cite{cgal:hk-bonp3-22b} or by a cut-cell meshing tools \cite{Tao:Mandoline:2019,Aftosmis:1998}, followed by a postprocessing to tesselate the interior of each cell with tetrahedra while ensuring a conforming mesh at the cell boundaries. 

We opted for a more direct and robust solution, creating a tetrahedral mesh of the bounding box of the surface mesh with fTetWild \cite{hu2020fast}, while providing explicit meshes of the regular grid as an additional input, which appear as triangular faces in the output mesh (Figure \ref{fig:teaser}). We then filter the tetrahedra outside the surface using the winding number \cite{Jacobson:2013}, and assign the resulting tetrahedra to the cell of the grid containing its barycenter. We use a geometrical tolerance of $10^{-3}$ for fTetWild.

To satisfy the minimum thickness requirement in 3D printing, the maximum size of the internal voids in boundary cells is restricted. However, some boundary cells might be too thin even without internal voids. If a thin boundary cell is adjacent to an interior cell, after the interior cell is replaced by the microstructure this boundary cell may violate the minimum thickness. To avoid this, we  change the type of some interior cells into boundary cells, although they are not cut by the boundary surface.  We compute the distance between the surface  cutting a boundary cell and its internal boundary faces,edges and vertices, shared with other internal cells; if the distance is too small, we transform all internal cells sharing this element into a boundary cell. 


\paragraph{Boundary-Cell Volumetric Meshing.}

In step 5, we need a second volumetric mesh, which is conforming to the geometry of the microstructure of inserted boundary cells.  This mesh is used for the second material optimization step (Section \ref{sec:optimization}), where the interior cells are further optimized to account for the error introduced by the mismatch of the actual properties of the boundary cells and the highly approximate homogeneous model we use for them at the first step. 

We also use fTetWild to create this mesh, using as an additional input the surface mesh of the microstructure of each boundary cell (Figure \ref{fig:teaser}).



\paragraph{Surface Extraction and Tunnels.}
\label{sec:tunnels}

To extract surfaces from implicit volumetric functions used both for internal cell microstructure definition and boundary cells,  we rely on the marching cube implementation in OpenVDB. We use a resolution of $50\times50\times50$ per cell (note that this effective resolution is used in a highly adaptive volumetric representation). . 

By construction, our boundary cells have a solid layer covering the model surface, that will prevent uncured resin or unmelted powder to be removed after fabricating the model. To make the model fabricable, we insert tunnels in each boundary cell. We first go over boundary cells with internal voids and consider the parts $B_E$ of their surfaces that belong to the outer surface. 
If for any point of $B_E$, the sphere of radius equal to the cylinder radius, intersects the  boundary curve of $B_E$, constructing a tunnel to the exterior is impossible, and we completely fill this  cell.   We create  cylinders connecting  the centers of every two adjacent boundary cells with voids; which form a graph consisting of disjoint connected components. 
For each such connected  component, we create a cylindrical tunnel from one void center to the object surface. To remove the materials inside interior cells, at least two tunnels are created from internal cells to adjacent boundary cells with voids. 

\paragraph{2D Pipeline.} 

Our 2D pipeline closely follows the 3D pipeline, using  triangle instead of fTetWild, and using our own implementation of marching squares as OpenVDB does not support 2D domains. An advantage of triangle is that it allows us to represent the boundaries exactly, without introducing a geometric approximation error. Tunnels are not added to the 2D boundary cells as they are not necessary for fabrication.






